On the Boltzmann Equation with Stochastic Kinetic Transport: Global Existence of Renormalized Martingale Solutions

This article studies the Cauchy problem for the Boltzmann equation with stochastic kinetic transport. Under a cut-off assumption on the collision kernel and a coloring hypothesis for the noise coefficients, we prove the global existence of renormalized (in the sense of DiPerna/Lions) martingale solutions to the Boltzmann equation for large initial data with finite mass, energy, and entropy. Our analysis includes a detailed study of weak martingale solutions to a class of linear stochastic kinetic equations. This study includes a criterion for renormalization, the weak closedness of the solution set, and tightness of velocity averages in $L^1$.

==> Compactness-and-Prelim-Renorm_Corollary-Proof.tex <==
%!TEX root = main.tex


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> Compactness-and-Prelim-Renorm_Velavg-Tightness.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

